Simple Kinesthetic Haptics for Object Recognition

Object recognition is an essential capability when performing various tasks. Humans naturally use either or both visual and tactile perception to extract object class and properties. Typical approaches for robots, however, require complex visual systems or multiple high-density tactile sensors which can be highly expensive. In addition, they usually require actual collection of a large dataset from real objects through direct interaction. In this paper, we propose a kinesthetic-based object recognition method that can be performed with any multi-fingered robotic hand in which the kinematics is known. The method does not require tactile sensors and is based on observing grasps of the objects. We utilize a unique and frame invariant parameterization of grasps to learn instances of object shapes. To train a classifier, training data is generated rapidly and solely in a computational process without interaction with real objects. We then propose and compare between two iterative algorithms that can integrate any trained classifier. The classifiers and algorithms are independent of any particular robot hand and, therefore, can be exerted on various ones. We show in experiments, that with few grasps, the algorithms acquire accurate classification. Furthermore, we show that the object recognition approach is scalable to objects of various sizes. Similarly, a global classifier is trained to identify general geometries (e.g., an ellipsoid or a box) rather than particular ones and demonstrated on a large set of objects. Full scale experiments and analysis are provided to show the performance of the method.

==> grasp_synthesis/exp.tex <==
\subsection{Grasp evaluation and synthesis}


\begin{itemize}
    \item
    Prediction accuracy - Confusion matrices. For different classifiers.
    \item
    2D grasps - plot Average computation time vs number of fingers. With and without friction.
    \item Number of force-closure solutions with regards to time - as in \cite{Watcharapol2015}. For each method, compare the discretization size of the friction cone with different curves. Several plots for 3-4 objects.
    \item
    Perhaps the same with bounded Q.
    \item
    Runtime of computing the quality measure.
    \item
    Compare the quality measure of the grasps.
\end{itemize}

==> grasp_synthesis/fundamentals.tex <==

In this section we briefly discuss grasping fundamentals that are used in this work. We present the common grasp model and discuss the notions of force-closure and grasp quality measure. We note that while we discuss spatial and planar objects in this paper, this section addresses the general case of spatial objects. The grasping fundamentals of planar objects can be easily deduced and are addressed in \cite{Sintov2014124}.

\subsection{Grasp Model}
Forces and torques can be represented as wrench vectors in the wrench space. In the spatial case, a wrench is a 6-dimensional vector and is denoted as $\vect{w}=(\vect{f}~~\vect{\tau})^{T}\in{}\mathbb{R}^6$  where $\vect{f}\in{}\mathbb{R}^3$ is the force vector and $\vect{\tau}\in{}\mathbb{R}^3$ is the torque vector. Furthermore, a wrench applied at contact point $\vect{p}_i\in\mathbb{R}^3$ relative to the object coordinate frame, can be described as $\vect{w}_i=(\vect{f}_i~~\vect{p}_i\times{\ve{f}_i})^{T}$. We model the friction between the fingertips of the gripper and the object's surface using the Coulomb model. In this model, forces exerted at the contact point must lie within a cone centered about the surface normal. This is known as the \textit{Friction Cone} (FC)
\begin{equation}
FC = \left\{\left( \begin{array}{c}
{f_{i,1}} \\
{f_{i,2}} \\
{f_{i,3}} \\
\end{array} \right):\left\vert\sqrt{{{f_{i,2}}}^2+{{f_{i,3}}}^2}\right\vert\leq \mu{}{f_{i,1}},~\forall{f_{i,1}}>0\right\}~~,
\end{equation}
where ${f_{i,1}}$ is the normal component of the force at the contact point, ${f_{i,2}}$ and ${f_{i,3}}$ are the tangential components, and $\mu$ is the coefficient of friction. The FC is non-linear and therefore can be approximated with an \textit{s}-sided convex polytope. Every force exerted within the FC can be represented by a linear combination of the unit vectors $\ve{\hat{f}}_{i,k}\in FC$ (the sign $\hat{.}$ denotes a unit vector) constructing the linearized friction cone (LFC), 
\begin{equation}
\label{eq:cone}
LFC=\left\{\vect{f_{i}}:\vect{f_{i}}=\sum_{k=1}^sa_{ik}\vect{\hat{f}}_{i,k},~a_{i,k}\geq0\right\}
\end{equation}
where $LFC\subset FC$ and $a_{i,k}$ is a non-negative coefficient \cite{Liu2000}.  The associated wrench can be expressed by
\begin{equation} 
\label{eq:wrench}
\vect{w}_{i}=\sum_{k=1}^sa_{i,k}\vect{\hat{w}}_{i,k}=\sum_{k=1}^sa_{i,k}\left( \begin{array}{c}
\vect{\hat{f}}_{i,k} \\
\vect{p}_i\times\vect{\hat{f}}_{i,k} \\
\end{array} \right)
\end{equation}
where $\vect{\hat{w}}_{i,k}$ are the primitive wrenches associated with the unit forces constructing the FC. 

An $n$-finger grasp of an object $\ssl{O}$ can be defined by a set of $n$ contact points, 
\begin{equation}
\ssl{P}=\left\{\vect{p_i}:\vect{p_i}\in\mathbb{R}^D~for~i=1,...,n\right\}
\label{eq:sslP}
\end{equation}
on the object's surface, and the normal to the object's surface at each point
\begin{equation}
\ssl{N}=\left\{\ve{n_i}:\ve{n_i}\in\mathbb{R}^D~for~i=1,...,n\right\},
\label{eq:sslN}
\end{equation}
where $\|\ve{n}_i\|=1$ and, $D=2$ or $D=3$ for planar and spatial objects, respectively. Equivalently, we can represent the grasp using the matching wrenches applied at the contact points $\ssl{\tilde{W}}=\left\{\ve{w}_1,...,\ve{w}_n\right\}$. If we consider friction, the wrench set can be expressed by the primitive wrenches 
\begin{equation}
\ssl{W}=\left\{\vect{w}_{1,1},\ve{w}_{1,2},...\ve{w}_{1,s},...,\ve{w}_{n,1},\ve{w}_{n,2},...,\ve{w}_{n,s}\right\}
\end{equation}
Using the above representation, we briefly describe the notion of a force closure grasp next.

\subsection{Force Closure}
A grasp is said to be force-closure if it is possible to apply wrenches at the contacts such that any external forces and torques acting on the object can be counter-balanced by the contact forces. In other words, a system of wrenches can achieve force-closure when they positively span the entire wrench space. Hence, any external load can be balanced by a non-negative combination of the wrenches \cite{Ponce1995}. According to \cite{Murray1994,Ponce1995,Mishra1987}, a necessary and sufficient condition for a system of wrenches $\ssl{W}$ to be force-closure is that the origin $O$ of $\mathbb{R}^6$ lies strictly in the interior of the \textit{Convex-Hull} (CH) of the contact primitive wrenches, i.e., 
\begin{equation}
    O\in{}interior(CH(\ssl{W}))
    \label{eq:interiorCH}
\end{equation}
where $O$ is the origin of the wrench space. Several algorithms exist for checking whether a set of wrenches $\ssl{W}$ satisfies condition \eqref{eq:interiorCH} \cite{Bailey1987}. Nevertheless, the common practice is described in \cite{Roa2009}. Briefly, let $H_k$ ($k=1,2,\ldots,n_f$) be a hyper-plane on the boundary of $CH(\ssl{W})$. The origin $O$ satisfies \eqref{eq:interiorCH} if and only if, for all $k$, any wrench $\ve{r}\in{}interior(CH(\ssl{W}))$ and $O$ lie in the same open half-space defined by $H_k$, i.e., lie on the same side of each of the convex hull's facets. By selecting $\ve{r}$ as a positive linear combination of the grasp wrenches, we can guarantee that it will constantly be in the interior of $CH(\ssl{W})$. 

The complexity of the Quickhull algorithm \cite{Bradford-Barber1996}, generally used for generation of convex-hulls, is in the order of $O(n_w \log(n_w))$, where $n_w$ is the number of wrenches forming the convex-hull. On top of that, the complexity of the force closure test is $O(n_f)$. The number $n_f$ of hyper-planes forming $CH(\ssl{W})$ can be large with the increase of contact points and unit vectors constructing their LFC.

\subsection{Grasp quality measure}

As mentioned above, a grasp that is force closure can resist external loads. A grasp quality measure quantifies how much a grasp can resist an external wrench without the fingers losing contact or starting to slip \cite{Borst1999}. A higher quality measure reduces object deformations due to contact force and actuator resources. The grasp quality measure is commonly used as a feasibility criterion and a selection tool to filter out unfitted grasps.

There are several known quality measures \cite{SDQM2017}. In general, the quality measure is the relation between wrenches that need to be applied and wrenches that can be applied. The most common quality measure is the largest ball criterion used when there is no prior knowledge of the task forces. In this method, the grasp quality is equivalent to the radius of the largest ball centered at the origin and fully contained in the $CH(\ssl{W})$ \cite{Roa2007}. In other words, the grasp quality measure is defined as the distance from the origin to the closest facet of the $CH(\ssl{W})$. Formally, we can say that the quality measure $Q$ is defined as
\begin{equation}
\label{eq:quality}
Q=\min_{\vect{w}\in \partial CH(\ssl{W})}\Vert \vect{w}\Vert
\end{equation}
where $\partial CH(\ssl{W})$ is the boundary of $CH(\ssl{W})$ \cite{Ferrari1992}. The quality measure in this method denotes the weakest net wrench that can be applied to counter-balance the external wrenches in its direction. In this work, we use this measure to demonstrate the proposed approach while others can similarly be used. 

  





==> grasp_synthesis/grasping.tex <==

In this section, we use the above grasp representation and propose an approach for rapid evaluation of grasps that can be applied to any object.

While the grasp parameterization described in the previous section is injective and independent of any coordinate system, it remains dependent of the objects size. That is, two objects of the same shape but with different size will have non-equal parameterization vector. Therefore, we would like to normalize the grasp such that objects of the same shape will have the same parameterization vector. Hence, we first define the scaling of a grasp representation.
\begin{mydef}
A grasp $\{\ssl{P},\ssl{N}\}$ is scaled by $k>0$ when its contact point coordinates are multiplied by $k$, i.e., the scaled grasp is given by $\{k\cdot\ssl{P},\ssl{N}\}$.
\end{mydef}
\noindent The above definition enables the scaling of the grasp size representation for further normalization. We now argue that scaling of a force-closure grasp maintains such property.
\begin{thm}
\label{thm:scaling}
A scaled grasp $\{k\cdot\ssl{P},\ssl{N}\}$ for $k > 0$ is force-closure, if grasp $\{\ssl{P},\ssl{N}\}$ is force-closure.
\end{thm}
\begin{proof}
Let $\ssl{W}$ be the wrenches of grasp $\{\ssl{P},\ssl{N}\}$ computed according to \eqref{eq:wrench}. The scaled grasp $\{k\cdot\ssl{P},\ssl{N}\}$ yields a wrench set $\tilde{\ssl{W}}$ such that any $\tilde{\ve{w}}\in\tilde{\ssl{W}}$ is given by
\begin{equation}
    \tilde{\ve{w}}=(\ve{f}~~(k\cdot\ve{p})\times{\ve{f}})^{T}=(\ve{f}~~k(\ve{p}\times{\ve{f}}))^{T}=K\ve{w},
\end{equation}
where $\ve{w}\in\ssl{W}$ and $K=\text{diag}(1,1,1,k,k,k)$ is a diagonal positive definite matrix. According to proposition 2.1 in \cite{Regis2016}, if the set $\ssl{W}=\{\ve{w}_1,\ldots,\ve{w_n}\}$ positively spans $\mathbb{R}^6$, then the set $\tilde{\ssl{W}}=\{K\ve{w}_1,\ldots,K\ve{w_n}\}$ for $K>0$ must also positively span $\mathbb{R}^6$. Hence, the scaled grasp $\{k\cdot\ssl{P},\ssl{N}\}$ is force-closure.
\end{proof}

Theorem \ref{thm:scaling} states that a force-closure grasp can be normalized by a scalar without losing the force-closure property. As mentioned, normalization should be done such that two objects of the same shape and with different size will have the same grasp parameterization vector. Hence, we normalize the grasp by scaling it by a size feature. A planar grasp represented by a polygon could be normalized by its circumference or area. Similarly, a spatial grasp polyhedron can be normalized by the sum of facet areas or edge lengths. Hence, given a grasp representation $\{\ssl{P},\ssl{N}\}$, its parameterization vector will be $\Phi\left(\{a_{\ssl{P}}^{-1}\cdot\ssl{P},\ssl{N}\}\right)$ where $a_{\ssl{P}}$ is the normalization scalar for $\ssl{P}$. It is important to note that, due to the normalization of the grasp representation, a grasp quality measure can now be compared between objects of different size. This could not have been done before since the torque elements of the wrenches in different size object are unequal.

To generate training data for classification and regression, one may sample grasps from a set of training objects and label them. However, such process will require many objects in order to get high variance in the data. Since the grasp parameterization is independent of any coordinate frame, we can sample vectors from $\mathbb{R}^D$.  We note that the bounds to sample from do not have much of importance since the samples are later normalized. For an $n$-finger grasp, we sample $n$ points in $\mathbb{R}^D$ to form $\ssl{P}_i$, generate the polygon (when $D=2$) or polyhedron (when $D=3$), and compute $a_{\ssl{P}_i}$. We then sample a unit vector for each vertex to generate $\ssl{N}_i$. Hence, we have sampled a normalized grasp representation $\{a_{\ssl{P}_i}\cdot\ssl{P}_i,\ssl{N}_i\}$ that can be mapped to $\ve{q}_i$. Vector $\ve{q}_i$ can be labeled by whether it is force-closure using \eqref{eq:interiorCH} or with its grasp quality measure (for example, using \eqref{eq:quality} when considering the largest ball criterion). This process is repeated until reaching the desired number of training samples and there is balanced representation of labeled data.

In this work, we use the generated training data to train a classifier to rapidly predict whether a sampled grasp from an object is force closure. Since we want to avoid the expensive generation of the convex-hull, we also train a regressor to approximate the quality measure of the grasp. The common approach to synthesize a grasp of an object is to sample possible grasps and to check for each, using \eqref{eq:interiorCH}-\eqref{eq:quality}, whether they are force-closure and have a quality measure above a lower bound. Using the classifier and regressor in a similar sampling process will enable faster synthesis of high-quality force-closure grasping postures.

